Giant Magnetocaloric Effect in Spin Supersolid Candidate Na$_2$BaCo(PO$_4$)$_2$

Supersolid, an exotic quantum state of matter that consists of particles forming an incompressible solid structure while simultaneously showing superfluidity of zero viscosity [1], is one of the long-standing pursuits in fundamental research [2, 3]. Although the initial report of $^4$He supersolid turned out to be an artifact [4], this intriguing quantum matter has inspired enthusiastic investigations into ultracold quantum gases [5-8]. Nevertheless, the realization of supersolidity in condensed matter remains elusive. Here we find evidence for a quantum magnetic analogue of supersolid -- the spin supersolid -- in the recently synthesized triangular-lattice antiferromagnet Na$_2$BaCo(PO$_4$)$_2$ [9]. Notably, a giant magnetocaloric effect related to the spin supersolidity is observed in the demagnetization cooling process, manifesting itself as two prominent valley-like regimes, with the lowest temperature attaining below 100 mK. Not only is there an experimentally determined series of critical fields but the demagnetization cooling profile also shows excellent agreement with the theoretical simulations with an easy-axis Heisenberg model. Neutron diffractions also successfully locate the proposed spin supersolid phases by revealing the coexistence of three-sublattice spin solid order and interlayer incommensurability indicative of the spin superfluidity. Thus, our results indicate a strong entropic effect of the spin supersolid phase in a frustrated quantum magnet and open up a viable and promising avenue for applications in sub-Kelvin refrigeration, especially in the context of persistent concerns about helium shortages [10, 11].

==> bibunits/README <==
Abstract

  The `bibunits' package allows separate bibliographies for different
  units or parts of the text. The units can be chapters, sections or
  bibunit environments. The package is compatible with a wide variety of
  packages, including, but not limited to, natbib, overcite and
  KOMA-SCRIPT classes.


To produce the style
  
  latex bibunits.ins


To produce the documentation

  latex bibunits.dtx

  If you do not want to include the macro section in the documentation,
  remove the comment sign before \OnlyDescription.


  To produce an index for the documentation:

    makeindex -s gind.ist bibunits

  To produce a change history for the documentation:
  
    makeindex -s gglo.ist -o bibunits.gls bibunits.glo


Contents:
 
  00Readme      this file ;-)
  bibunits.dtx  documented source file for the bibunits package
  bibunits.ins  installation file
  bibtexall     shell script to run bibtex on each .aux file in the
                   present directory


License

  Package `bibunits' to use with LaTeX2e.

  Copyright (C) 1999--2004 Thorsten Hansen

  This work may be distributed and/or modified under the conditions of
  the LaTeX Project Public License, either version 1.3 of this license
  or any later version. The latest version of this license is in
  http://www.latex-project.org/lppl.txt and version 1.3 or later is
  part of all distributions of LaTeX version 2003/12/01 or
  later.
  
  This work has the LPPL maintenance status "maintained". The Current
  Maintainer of this work is Thorsten Hansen.
  
  This work consists of the files bibunits.dtx and bibunits.ins
  and the derived file bibunits.sty.




Happy TeXing

    Thorsten Hansen
    thorsten.hansen@psychol.uni-giessen.de

